CODA: A Continuous Online Evolve Framework for Deploying HAR Sensing Systems

In always-on HAR deployments, model accuracy erodes silently as domain shift accumulates over time. Addressing this challenge requires moving beyond one-off updates toward instance-driven adaptation from streaming data. However, continuous adaptation exposes a fundamental tension: systems must selectively learn from informative instances while actively forgetting obsolete ones under long-term, non-stationary drift. To address them, we propose CODA, a continuous online adaptation framework for mobile sensing. CODA introduces two synergistic components: (i) Cache-based Selective Assimilation, which prioritizes informative instances likely to enhance system performance under sparse supervision, and (ii) an Adaptive Temporal Retention Strategy, which enables the system to gradually forget obsolete instances as sensing conditions evolve. By treating adaptation as a principled cache evolution rather than parameter-heavy retraining, CODA maintains high accuracy without model reconfiguration. We conduct extensive evaluations on four heterogeneous datasets spanning phone, watch, and multi-sensor configurations. Results demonstrate that CODA consistently outperforms one-off adaptation under non-stationary drift, remains robust against imperfect feedback, and incurs negligible on-device latency.

==> 0abstract.tex <==

\begin{abstract}
In recent years, emerging research on mobile sensing presents a good variety of novel scenarios that benefit human daily life. 
However, dynamic usage conditions regarding diverse users and devices result in performance degradation when systems are deployed in the wild. 
Existing solutions mainly address the problem with a one-off adaptation scheme based on a neural network which is hard to guarantee robustness against uncertain drifting conditions in human-centric sensing scenarios (e.g. activity of daily life recognition, gesture recognition).  
In this paper, we review the problem from the instance-level data distribution perspective and develop CODA, a continuous online adaptation framework for mobile sensing. 
Built upon a cache-like structure, CODA integrates the importance weighted active learning and further guarantees effective adaptation with a retentive weighting strategy. 
A series of evaluations across four datasets, covering phone-based, watch-based and integrated sensors-based sensing tasks, further demonstrate the feasibility as well as the potential in online adaptation with CODA. 
The promising results by CODA (even without learnable parameters) also indicate the possibility of the realization of unobtrusive adaptation with sufficient feedback by some specific application designs.
\end{abstract}

==> 2related_work.tex <==

\section{Related Work}\label{section:background}

% In this section, we investigate the idea in developing the mechanism for adapting online by first introducing existed solutions for domain adaptation.
% Depicting the potential in adaptation online, we then illustrate the basic idea in integrating active learning into our design. 
% In the later part of the section, we further introduce the idea in benchmarking the online adaptation scenarios, targeting on showing the intrinsic difference from traditional domain adaptation.

\subsection{HAR in Always-On Mobile Sensing Systems}
Human activity recognition (HAR) has become a core sensing primitive in a wide range of always-on applications, including healthcare monitoring\cite{chen2019taprint, pan2025cgmm}, assisted living\cite{kim2024iris,thukral2025layout, teng2023pdges}, and fall detection\cite{waffle, wang2016wifall}.
Unlike controlled experimental settings, real-world HAR systems operate continuously under evolving users, device configurations, and environmental conditions~\cite{chen2021deep},
inevitably inducing distribution shifts between training and deployment data~\cite{yoon2025selfreplay,stisen_smart_2015, ustev2013user}.
Thus, models that perform well in controlled settings often suffer substantial performance degradation after deployment~\cite{ min_early_2019,yang_toward_2009,ustev2013user}.


% Early HAR approaches primarily relied on conventional classifiers \cite{ramasamy2018recent}.
% Recent years, deep learning architectures have become increasingly prevalent due to their ability to automatically learn spatiotemporal representations from raw sensor data, leading to substantial performance improvements\cite{chen2021deep}.
% Most existing HAR systems, however, implicitly assume that activity-specific patterns remain distinctive and stable across users, devices, and environments, and can be reliably characterized using variant sensor measurements.
% In practice, this assumption is frequently violated.
% Variations in sensor placement, user biomechanics, device hardware, and time-dependent sensor drift can substantially distort these patterns, resulting in distribution shifts between training and deployment data\cite{yoon2025selfreplay,stisen_smart_2015, ustev2013user}.
% As a consequence, HAR models that perform well under controlled settings often experience significant performance degradation in real-world environments\cite{weiss_impact_nodate, min_early_2019,yang_toward_2009,ustev2013user}.
% Ensuring robustness under such distributional heterogeneity remains a central and largely unresolved challenge in sensor-based HAR research.


\subsection{Domain Adaptation Techniques}
To mitigate performance degradation caused by domain shift, numerous domain adaptation and generalization methods have been proposed.
Broadly, existing approaches fall into three categories: data-level operations, representation learning, and learning strategies.
Data-level methods improve generalization by manipulating training data to better cover potential target domains \cite{lee2025domclp}.
These methods assume that domain discrepancies can be alleviated by reshaping or enriching the training data distribution.
Representation learning approaches focus on learning domain-invariant features through feature alignment or invariant network designs\cite{qin2022domain, cheng2024disentangled, yu2024clipceil}.
Learning strategy–based methods, including meta-learning and ensemble learning, leverage prior knowledge to improve adaptation efficiency \cite{gong_metasense_2019, yoon2025selfreplay}.
Recent HAR studies further integrate meta-learning with self-supervised objectives, such as CrossHAR and ContrastSense, to enhance cross-dataset generalization under limited labels\cite{lu2022semantic, qian2021latent, qin2022domain, hong2024crosshar, dai2024contrastsense}.
\textit{Despite their effectiveness, 
these methods largely rely on an episodic adaptation paradigm, in which adaptation is performed as a one-off process under the assumption of a well-defined target domain or a finite adaptation stage.
Such assumptions fundamentally break down in real-world mobile sensing deployments, where domain drift emerges continuously and unpredictably over time.}

% In contrast, our work focuses on sustained, deployment-time adaptation, enabling mobile sensing systems to evolve continuously with minimal supervision and low operational cost.



% \subsection{Necessity of Receiving Feedback}
% % Q1- What I do to address this problem?
% % A: with little controled, self-collected datasets
% To further address the challenge of driftings in practical usage, we simulate two different types of scenarios (TAPRINT for gesture recognition and WHAR for human activity recognition) and have the data collected with minimum control on the user behaviors. 
% % Q2- How to show the drifting?
% % A: Isomap
% We further inspect the data distributions by adopting Isomap \cite{}, a visualization technique that helps retain the global structure of data in the high dimensional space, and observe the driftings along the time on both datasets.
% % Q3- What messages in the figure?
% % A1: distribution driftings
% % A2: unsolvable driftings
% The figures \ref{xxx} shows two typical driftings on different tasks respectively.
% We also compare the variance in features. 
% In addition to the hand-tune features (selected by cross validation), we further reimplement MetaSense\cite{gong_metasense_2019}, a meta-learning based domain adaptation technique for human activity recognition, and generate the augmented features with a trained neural network model (detailed settings in section \ref{}).

% % TODO: should I extend the discussion about meta sense?
% In general, we show that such kind of driftings is unsolvable by one-off adaptation, at least not now with only few initial data from the user, which makes it quite challenging to maintain the robustness of a system.
% So the intuitive solution is to get informed during the usage and retrain the model in time. 
% However, it could be both time and memory consuming to retrain a model with sufficient data.
% The uncertainty inherited in a model might be no less than that in driftings.
% Overfitting and underfitting are two popular problems that we could still often meet in training a data-hungry model with just few data today\cite{}.





% \subsection{Promising Online Adaptation}
% In this paper, we further notice the fact that in different periods of usage, the instances with same label gather as a cluster and instances from different labels are still distinguishable even after the driftings.
% This observation of clustering phenomenon motivates the adoptation of the simple and mature classifier of K Nearest Neighbors, which works in a way of matching the patterns and doesn't require explicit training process.

% \subsubsection{Evidence in Performance}
% 1. online conditions are drifting in the wild.
% 2. 
% The needs for continuous adaptation could be dated back to even last 90s. 
% To quantify the gap by 
% How to show the evidence ?
% 1- 4 datasets (2 self-collected and 2 public)
% 2- baseline preparation
%   logic here:
%     2.1- what?
%           validation with Nearest Neighbor model
%           KNN and MetaSense - one-off domain adaptation setting
%     2.2- why?
%           - MetaSense injects the prior knowledge about variance from 
%             the collections in other conditions.
%           - KNN is too simple to obtain high performance in one-off 
%             adaptaion.
%           - Comparing to the one-off adaptaion, cross validation shows
%             the potential by introducing the online adaptation setting 
%             even with the simple Nearest Neighbor model. 
%           - To some extend, the validation result also serves as the 
%             near optimal performance for the Nearest Neighbor model 
%             with no limitation in the storage.
% We further demonstrate the feasibility with experiments on 4 mobile sensing datasets (2 self-collected and 2 public datasets), and the results are summarized in figure~\ref{fig:exp_0_motivation}.
% We first implement the KNN (K is empirically set to 5) and MetaSense (implementation details in section ~\ref{}) in one-off domain adaptation setting.
% As expected, the MetaSense does assimilate some prior knowledge from the other collections, takes advantage of neural network model, and therefore achieves higher performance than KNN model.
% We then compare the one-off domain adaptation baselines with the cross validation. 
% Particularly, the cross validation is implemented with the rather weaker model of Nearest Neighbors based on some domain-specific metric, and the difference to the one-off adaptation setting is that the validation assumes the availability of the instances on the fly.
% Generally speaking, the surpassing performance of cross-validation further demonstrates the potential of having online feedback exposed to the even simple model.


% \subsubsection{Periodic Clustering Opportunity} 
% What ?
%   - How to avoid the impact by collision? 
%     - whether it is a problem?
%     - [x] 1. validate it with the performance ? --> too complex
%     - [x] 2. comparing it with the difference by driftings ?
%     - No it might not be a problem to be solved,
% The validation result shows the potential in utilizing the online feedback data by a similarity-based 
% mechanisms, while also addresses concerns about the requirements of the data.
% Especially for a similarity-based model, 
% As a model based on pattern matching, the Knn is famous for its flexibility.
%     
%     
% How ?
%     what caching account for?
%     how expired instances influence the performance ?
%     - function like a cache, eliminate the expired instances.
% As we mentioned in the early section that KNN is a rather simple model with the interesting character of working without training. 
% Precisely, the KNN functions in a way of matching the testing pattern to the candidates stored in a database, and any modification (like append, remove, .etc) on the database could result in different performance.
% But it is also blamed for the 'laziness' in learning from the data. 
% One of the related drawbacks could be the linear complexity on the number of instances.
% % TODO: conventional solution to solve this problem ?
% % 
% While recapturing the driftings observed in the usage data, we show the clustering tends to remain stable in the period they belong to. 
% It actually implies the possibility in guaranteeing performance with just a small amount of data which further motivates the cache-like design on the database utilized for classification.
% In particular, the system only allows replacement action upon the database to maintain the candidates number as well as the efficiency (e.g. the classification delay time) along with the usage. 
% \subsubsection{More Effective Replacement Strategy} 
% % why we need efficient strategy?
% % how active learning can help ?
% % what is the difference?
% Motivating by the observations on the dynamicity of the usage, we decide to explore the potential by KNN model with a cache-like database refreshing the candidates simultaneously. 
% Modification on the set of candidates could result in different performance, but what is a better strategy remains ambiguous. 
% Some ideas could be quite heuristic. 
% For example, based on the time sensitive motivation, we can just define the relative arrival time till the present as the metric about expiration (refers to the TimeHeuristics mentioned in the section~\ref{}).
% % based on the distance
% Another strategy can be based on a clustering idea. Particularly, we can replace the instance that is most dissimilar to the latest instance with feedback.
% Or we can also devalue the selection of the instance to be replaced, since the latest instance contributes the main improvement in the performance according to the motivation.
% Indeed, we can also devalue the selection process and just do a random replacement, since the latest instance contributes the main improvement in the performance according to the motivation.
% An efficient strategy of random replacement devalues the selection of the instances to be replaced but addresses 
% 
% lack of connection to the KNN model.
%   Why conncetion to the KNN model is important ?
% The challenge in designing an efficient strategy is that different metrics sometimes can result in similar selection.
% However, it is actually hard to tell which strategy is the best because their metrics can result in some similar selections and even performance as well.
% We believe a more effective strategy should address the connection 
% between the replacements and the KNN model.
% Precisely, we introduce Importance Weighted Active Learning~\cite{beygelzimer_importance_2009} that is originally proposed to train a binary classifier with limited amount of samples efficiently.
% Different from other heuristic active learning criterion\cite{settles2009active} (e.g. uncertainty, diversity, .etc), this mechanism provides an importance evaluation framework on the instances based on some loss specified for the target model.
% % explaining how active learning contributes the algorithm design ...
% %   a theorem that helps explain the selection with loss.
% %     How ?
% %       - loss design ?
% %       - periodic importance ?
% In CODA, we design a clustering loss that aims at regularizing the relationships between classes and enable more effective multi-class classification with KNN model.
% % Based on the observations of the drifting distributions, a memory retentive weighting strategy is introduced to make sure the evaluation more precise.
% Additionally, based on the observations of the drifting distributions, a memory retentive weighting strategy is further introduced to guarantee the evaluation follows the latest interest.

% \subsubsection{Benchmarking the Online Adaptation}
% Online adaptation is apparently different from the traditional domain adaptation task 
% The experiments design mainly emphasize the generality of adaptation with CODA by variant settings.
% What ?
%  In this paper, we address the logic in experiment designs...
% Why ?
% 
% The online setting is introduced 

% To validate the performance of the online adaptation, the experiment designs are of the vital importance while remains challenging.
% To begin with, in this paper, we reimplement conventional one-off setting of adaptation on 4 datasets (section~\ref{subsec:dataSets} and ~\ref{subsec:pilotStudy}).
% After showing the promising improvements by online setting (section~\ref{subsec:ODA}), a series of novel and bold settings (Target Agnostic in section~\ref{subsec:TAD} and Long-term Adaptation in section ~\ref{subsec:longtermDA}) are evaluated as well.
% We further investigate the reliance on the feedback ratio (section~\ref{subsec:practicalAd}) and conclude the discussion with system performance (section~\ref{subsec:impl}).


==> append_exp/new_table/2022_Exp_longterm_sum.tex <==
\begin{table}[htbp]
\centering
\caption{Long-term experiments inspected with smartwatches.}
\label{tab:longterm_sum}
\begin{tabular}{lcccccc}
\toprule
{} & \multicolumn{2}{c}{LG} & \multicolumn{2}{c}{HW} & \multicolumn{2}{c}{TW} & {mean} \\
{} & {WHAR} & {TAPRINT} & {WHAR} & {TAPRINT} & {WHAR} & {TAPRINT} & {} \\
\midrule
5NN & \color{gray} \underline 0.3497 & \color{gray} \underline 0.3076 & \color{gray} \underline 0.3642 & \color{gray} \underline 0.2634 & \color{gray} \underline 0.3650 & \color{gray} \underline 0.3559 & \color{gray} \underline 0.3343 \\
RND & 0.8304 & 0.7888 & 0.8625 & 0.7424 & 0.8019 & 0.6918 & 0.7863 \\
TH & \color{gray} \underline 0.8133 & \color{black} 0.7972 & \color{gray} \underline 0.8328 & \color{black} 0.7470 & \color{gray} \underline 0.7875 & \bfseries \color{black} 0.7071 & \color{gray} \underline 0.7808 \\
CODA_B & \color{gray} \underline 0.5575 & \color{gray} \underline 0.7103 & \color{gray} \underline 0.5678 & \color{gray} \underline 0.6395 & \color{gray} \underline 0.4894 & \color{gray} \underline 0.5721 & \color{gray} \underline 0.5894 \\
CODA_L & \color{gray} \underline 0.8219 & \color{gray} \underline 0.7844 & \color{gray} \underline 0.8563 & \color{black} 0.7459 & \color{black} 0.8133 & \color{black} 0.6946 & \color{gray} \underline 0.7860 \\
CODA & \bfseries \color{black} 0.8460 & \bfseries \color{black} 0.7991 & \bfseries \color{black} 0.8687 & \bfseries \color{black} 0.7545 & \bfseries \color{black} 0.8197 & \color{black} 0.6949 & \bfseries \color{black} 0.7971 \\
\bottomrule
\end{tabular}
\end{table}


==> append_exp/new_table/2022_exp_5_4_longterm_sum_in_MFR_50_40_.tex <==
\begin{table}[htbp]
\centering
\caption{Long-term experiments inspected with smartwatches.}
\label{tab:longterm_sum}
\begin{tabular}{lcccccc}
\toprule
{} & \multicolumn{2}{c}{LG} & \multicolumn{2}{c}{HW} & \multicolumn{2}{c}{TW} & {mean} \\
{} & {WHAR} & {TAPRINT} & {WHAR} & {TAPRINT} & {WHAR} & {TAPRINT} & {} \\
\midrule
5NN & \color{gray} \underline 0.3497 & \color{gray} \underline 0.3076 & \color{gray} \underline 0.3642 & \color{gray} \underline 0.2634 & \color{gray} \underline 0.3650 & \color{gray} \underline 0.3559 & \color{gray} \underline 0.3343 \\
RND & 0.6538 & 0.6774 & 0.6497 & 0.6509 & 0.6166 & 0.5603 & 0.6348 \\
TH & \color{gray} \underline 0.5810 & \color{black} 0.6818 & \color{gray} \underline 0.6229 & \color{gray} \underline 0.6421 & \color{gray} \underline 0.6117 & \color{black} 0.5677 & \color{gray} \underline 0.6179 \\
CODA-P & \color{gray} \underline 0.6016 & \color{gray} \underline 0.6406 & \color{gray} \underline 0.5314 & \color{gray} \underline 0.5033 & \color{gray} \underline 0.5458 & \color{gray} \underline 0.4887 & \color{gray} \underline 0.5519 \\
CODA-L & \color{gray} \underline 0.6292 & \color{gray} \underline 0.6673 & \color{black} 0.7096 & \color{black} 0.6529 & \color{gray} \underline 0.6147 & \color{black} 0.5841 & \color{black} 0.6430 \\
CODA & \bfseries \color{black} 0.7446 & \bfseries \color{black} 0.7051 & \bfseries \color{black} 0.7657 & \bfseries \color{black} 0.6535 & \bfseries \color{black} 0.7350 & \bfseries \color{black} 0.5848 & \bfseries \color{black} 0.6981 \\
\bottomrule
\end{tabular}
\end{table}


==> figs/figs_tables/output_tables/0_feature_selection.tex <==
\begin{table}[h]
\centering
\caption{Feature Selection Results}
\label{tab:featSelection}
\begin{tabular}{rrrrr}
\toprule
{} & {} & {PAMAP2} & {HHAR} & {WHAR} & {TAPRINT} \\
\midrule
\multirow[t]{2}{*}{raw} & euclidean & 0.8277 & 0.7451 & 0.7721 & 0.7657 \\
 & dtw & 0.8539 & 0.7014 & 0.6592 & \itshape \bfseries 0.7863 \\
ecdf & euclidean & \itshape \bfseries 0.8828 & \itshape \bfseries 0.8980 & \itshape \bfseries 0.8727 & 0.6856 \\
\bottomrule
\end{tabular}
\end{table}


==> figs/figs_tables/output_tables/1_detailed_result.tex <==
\begin{table}[h]
\centering
\caption{Detailed Results For One-time Adaptation Baselines}
\label{tab:detailedRst}
\begin{tabular}{rrrrr}
\toprule
{} & {PAMAP2} & \multicolumn{3}{r}{HHAR} & \multicolumn{3}{r}{WHAR} & \multicolumn{3}{r}{TAPRINT} \\
{} & {-} & {$nexus4^*$} & {s3} & {samsungold} & {$HW^*$} & {TW} & {LG} & {HW} & {TW} & {LG} \\
\midrule
CrossValid. & \itshape \bfseries 0.8828 & \itshape \bfseries 0.9168 & \itshape \bfseries 0.8896 & \itshape \bfseries 0.8875 & \itshape \bfseries 0.8972 & \itshape \bfseries 0.8648 & \itshape \bfseries 0.8561 & \itshape \bfseries 0.7562 & \itshape \bfseries 0.7619 & \itshape \bfseries 0.8410 \\
5NN & 0.1169 & 0.8095 & 0.7889 & 0.6757 & 0.5173 & 0.5689 & 0.5187 & 0.5197 & 0.4408 & 0.5717 \\
MetaSense & 0.6327 & 0.8565 & 0.8594 & 0.7313 & 0.7790 & 0.7850 & 0.7921 & 0.6499 & 0.5407 & 0.6821 \\
\bottomrule
\end{tabular}
\end{table}


==> figs/figs_tables/output_tables/4_1_cross_user_rst.tex <==
\begin{table}[h]
\centering
\caption{Impacts By Crossing Explicit Conditions of Users}
\label{tab:crossUser}
\begin{tabular}{rrrrr}
\toprule
{} & {} & {HHAR} & {WHAR} & {TAPRINT} \\
\midrule
\multirow[t]{3}{*}{$DA^\ast$} & 5NN & 0.8457 & 0.5173 & 0.5107 \\
 & MetaSense & 0.8937 & 0.7790 & 0.6242 \\
 & CrossValid. & 0.9104 & 0.8972 & 0.7863 \\
\multirow[t]{2}{*}{w/o DA} & 5NN & \underline \bfseries 0.3587 & \underline \bfseries 0.3299 & \underline \bfseries 0.1924 \\
 & MetaSense & 0.3716 & 0.5027 & 0.2164 \\
\bottomrule
\end{tabular}
\end{table}


==> figs/figs_tables/output_tables/4_2_cross_model_rst.tex <==
\begin{table}[h]
\centering
\caption{Impacts By Crossing Explicit Conditions of Models}
\label{tab:crossModel}
\begin{tabular}{rrrrr}
\toprule
{} & {} & {HHAR} & {WHAR} & {TAPRINT} \\
\midrule
\multirow[t]{3}{*}{$DA^\ast$} & 5NN & 0.8066 & 0.5350 & 0.5107 \\
 & MetaSense & 0.8748 & 0.7854 & 0.6242 \\
 & CrossValid. & 0.9000 & 0.8727 & 0.7863 \\
\multirow[t]{2}{*}{w/o DA} & 5nn & \underline \bfseries 0.6973 & \underline \bfseries 0.5325 & 0.3219 \\
 & MetaSense & 0.7206 & 0.7141 & \underline \bfseries 0.2378 \\
\bottomrule
\end{tabular}
\end{table}


==> figs/n_tables/Exp_longterm_sum.tex <==
\begin{table}[htbp]
\centering
\caption{Long-term experiments inspected with smartwatches.}
\label{tab:longterm_sum}
\begin{tabular}{lcccccc}
\toprule
{} & \multicolumn{2}{c}{HW} & \multicolumn{2}{c}{TW} & \multicolumn{2}{c}{LG} & {mean} \\
{} & {WHAR} & {TAPRINT} & {WHAR} & {TAPRINT} & {WHAR} & {TAPRINT} & {} \\
\midrule
5NN & \color{gray} \underline 0.3642 & \color{gray} \underline 0.2634 & \color{gray} \underline 0.3650 & \color{gray} \underline 0.3559 & \color{gray} \underline 0.3497 & \color{gray} \underline 0.3076 & \color{gray} \underline 0.3343 \\
RND & 0.8625 & 0.7424 & 0.8019 & 0.6918 & 0.8304 & 0.7888 & 0.7863 \\
TH & \color{gray} \underline 0.8328 & \color{black} 0.7470 & \color{gray} \underline 0.7875 & \bfseries \color{black} 0.7071 & \color{gray} \underline 0.8133 & \bfseries \color{black} 0.7972 & \color{gray} \underline 0.7808 \\
CODA_B & \color{gray} \underline 0.5740 & \color{gray} \underline 0.6395 & \color{gray} \underline 0.5230 & \color{gray} \underline 0.5721 & \color{gray} \underline 0.5610 & \color{gray} \underline 0.7103 & \color{gray} \underline 0.5967 \\
CODA_L & \color{gray} \underline 0.8563 & \color{black} 0.7459 & \color{black} 0.8133 & \color{black} 0.6946 & \color{gray} \underline 0.8219 & \color{gray} \underline 0.7844 & \color{gray} \underline 0.7860 \\
CODA & \bfseries \color{black} 0.8644 & \bfseries \color{black} 0.7474 & \bfseries \color{black} 0.8291 & \color{black} 0.6995 & \bfseries \color{black} 0.8505 & \color{black} 0.7969 & \bfseries \color{black} 0.7980 \\
\bottomrule
\end{tabular}
\end{table}


==> figs/n_tables/exp_5_3_longterm_sum.tex <==
\begin{table}[htbp]
\centering
\caption{Long-term experiments inspected with smartwatches.}
\label{tab:longterm_sum}
\begin{tabular}{lcccccc}
\toprule
{} & \multicolumn{2}{c}{HW} & \multicolumn{2}{c}{TW} & \multicolumn{2}{c}{LG} \\
{} & {WHAR} & {TAPRINT} & {WHAR} & {TAPRINT} & {WHAR} & {TAPRINT} \\
\midrule
5NN & \color{gray} \underline 0.3642 & \color{gray} \underline 0.2634 & \color{gray} \underline 0.3650 & \color{gray} \underline 0.3559 & \color{gray} \underline 0.3497 & \color{gray} \underline 0.3076 \\
RND & 0.7230 & 0.6509 & 0.6954 & 0.5603 & 0.6603 & 0.6774 \\
TH & \color{gray} \underline 0.6560 & \color{gray} \underline 0.6421 & \color{gray} \underline 0.6746 & \color{black} 0.5677 & \color{gray} \underline 0.6207 & \color{black} 0.6818 \\
CODA-P & \color{gray} \underline 0.5232 & \color{gray} \underline 0.5033 & \color{gray} \underline 0.5607 & \color{gray} \underline 0.4887 & \color{gray} \underline 0.5379 & \color{gray} \underline 0.6406 \\
CODA-L & \color{black} 0.7274 & \color{black} 0.6529 & \color{black} 0.6989 & \bfseries \color{black} 0.5841 & \color{black} 0.6668 & \color{gray} \underline 0.6673 \\
CODA & \bfseries \color{black} 0.8165 & \bfseries \color{black} 0.6539 & \bfseries \color{black} 0.8004 & \color{black} 0.5769 & \bfseries \color{black} 0.7772 & \bfseries \color{black} 0.7019 \\
\bottomrule
\end{tabular}
\end{table}


==> figs/n_tables/exp_5_4_longterm_sum_in_MFR_60_40_.tex <==
\begin{table}[htbp]
\centering
\caption{Long-term experiments inspected with smartwatches.}
\label{tab:longterm_sum}
\begin{tabular}{lcccccc}
\toprule
{} & \multicolumn{2}{c}{HW} & \multicolumn{2}{c}{TW} & \multicolumn{2}{c}{LG} & {mean} \\
{} & {WHAR} & {TAPRINT} & {WHAR} & {TAPRINT} & {WHAR} & {TAPRINT} & {} \\
\midrule
5NN & \color{gray} \underline 0.3642 & \color{gray} \underline 0.2634 & \color{gray} \underline 0.3650 & \color{gray} \underline 0.3559 & \color{gray} \underline 0.3497 & \color{gray} \underline 0.3076 & \color{gray} \underline 0.3343 \\
RND & 0.7230 & 0.6509 & 0.6954 & 0.5603 & 0.6603 & 0.6774 & 0.6612 \\
TH & \color{gray} \underline 0.6560 & \color{gray} \underline 0.6421 & \color{gray} \underline 0.6746 & \color{black} 0.5677 & \color{gray} \underline 0.6207 & \color{black} 0.6818 & \color{gray} \underline 0.6405 \\
CODA-P & \color{gray} \underline 0.5232 & \color{gray} \underline 0.5033 & \color{gray} \underline 0.5607 & \color{gray} \underline 0.4887 & \color{gray} \underline 0.5379 & \color{gray} \underline 0.6406 & \color{gray} \underline 0.5424 \\
CODA-L & \color{black} 0.7274 & \color{black} 0.6529 & \color{black} 0.6989 & \bfseries \color{black} 0.5841 & \color{black} 0.6668 & \color{gray} \underline 0.6673 & \color{black} 0.6662 \\
CODA & \bfseries \color{black} 0.8165 & \bfseries \color{black} 0.6539 & \bfseries \color{black} 0.8004 & \color{black} 0.5769 & \bfseries \color{black} 0.7772 & \bfseries \color{black} 0.7019 & \bfseries \color{black} 0.7211 \\
\bottomrule
\end{tabular}
\end{table}


==> figs/n_tables/exp_5_4_longterm_sum_in_TAFR_70_70_.tex <==
\begin{table}[htbp]
\centering
\caption{Long-term experiments inspected with smartwatches.}
\label{tab:longterm_sum}
\begin{tabular}{lcccccc}
\toprule
{} & \multicolumn{2}{c}{HW} & \multicolumn{2}{c}{TW} & \multicolumn{2}{c}{LG} & {mean} \\
{} & {WHAR} & {TAPRINT} & {WHAR} & {TAPRINT} & {WHAR} & {TAPRINT} & {} \\
\midrule
5NN & \color{gray} \underline 0.3642 & \color{gray} \underline 0.2634 & \color{gray} \underline 0.3650 & \color{gray} \underline 0.3559 & \color{gray} \underline 0.3497 & \color{gray} \underline 0.3076 & \color{gray} \underline 0.3343 \\
RND & 0.7599 & 0.7065 & 0.7221 & 0.6521 & 0.7521 & 0.7542 & 0.7245 \\
TH & \color{gray} \underline 0.6862 & \color{black} 0.7134 & \color{black} 0.7375 & \color{black} 0.6601 & \color{gray} \underline 0.6964 & \bfseries \color{black} 0.7667 & \color{gray} \underline 0.7101 \\
CODA-P & \color{gray} \underline 0.5534 & \color{gray} \underline 0.6305 & \color{gray} \underline 0.5255 & \color{gray} \underline 0.5293 & \color{gray} \underline 0.5324 & \color{gray} \underline 0.6920 & \color{gray} \underline 0.5772 \\
CODA-L & \color{gray} \underline 0.7432 & \color{black} 0.7149 & \color{black} 0.7390 & \color{gray} \underline 0.6506 & \color{gray} \underline 0.7346 & \color{gray} \underline 0.7514 & \color{gray} \underline 0.7223 \\
CODA & \bfseries \color{black} 0.8189 & \bfseries \color{black} 0.7175 & \bfseries \color{black} 0.8024 & \bfseries \color{black} 0.6707 & \bfseries \color{black} 0.8123 & \color{black} 0.7623 & \bfseries \color{black} 0.7640 \\
\bottomrule
\end{tabular}
\end{table}


==> figs/output_tables/0_feature_selection.tex <==
\begin{table}[h]
\centering
\caption{Feature Selection Results}
\label{tab:featSelection}
\begin{tabular}{rrrrr}
\toprule
{} & {} & {PAMAP2} & {HHAR} & {WHAR} & {TAPRINT} \\
\midrule
\multirow[t]{2}{*}{raw} & euclidean & 0.8277 & 0.7451 & 0.7721 & 0.7657 \\
 & dtw & 0.8539 & 0.7014 & 0.6592 & \itshape \bfseries 0.7863 \\
ecdf & euclidean & \itshape \bfseries 0.8828 & \itshape \bfseries 0.8980 & \itshape \bfseries 0.8727 & 0.6856 \\
\bottomrule
\end{tabular}
\end{table}


==> figs/output_tables/1_detailed_result.tex <==
\begin{table}[h]
\centering
\caption{Detailed Results For One-time Adaptation Baselines}
\label{tab:detailedRst}
\begin{tabular}{rrrrr}
\toprule
{} & {PAMAP2} & \multicolumn{3}{r}{HHAR} & \multicolumn{3}{r}{WHAR} & \multicolumn{3}{r}{TAPRINT} \\
{} & {-} & {$nexus4^*$} & {s3} & {samsungold} & {$HW^*$} & {TW} & {LG} & {HW} & {TW} & {LG} \\
\midrule
CrossValid. & \itshape \bfseries 0.8828 & \itshape \bfseries 0.9168 & \itshape \bfseries 0.8896 & \itshape \bfseries 0.8875 & \itshape \bfseries 0.8972 & \itshape \bfseries 0.8648 & \itshape \bfseries 0.8561 & \itshape \bfseries 0.7562 & \itshape \bfseries 0.7619 & \itshape \bfseries 0.8410 \\
5NN & 0.1169 & 0.8095 & 0.7889 & 0.6757 & 0.5173 & 0.5689 & 0.5187 & 0.5197 & 0.4408 & 0.5717 \\
MetaSense & 0.6327 & 0.8565 & 0.8594 & 0.7313 & 0.7790 & 0.7850 & 0.7921 & 0.6499 & 0.5407 & 0.6821 \\
\bottomrule
\end{tabular}
\end{table}


==> figs/output_tables/4_1_cross_user_rst.tex <==
\begin{table}[h]
\centering
\caption{Impacts By Crossing Explicit Conditions of Users}
\label{tab:crossUser}
\begin{tabular}{rrrrr}
\toprule
{} & {} & {HHAR} & {WHAR} & {TAPRINT} \\
\midrule
\multirow[t]{3}{*}{$DA^\ast$} & 5NN & 0.8457 & 0.5173 & 0.5107 \\
 & MetaSense & 0.8937 & 0.7790 & 0.6242 \\
 & CrossValid. & 0.9104 & 0.8972 & 0.7863 \\
\multirow[t]{2}{*}{w/o DA} & 5NN & \underline \bfseries 0.3587 & \underline \bfseries 0.3299 & \underline \bfseries 0.1924 \\
 & MetaSense & 0.3716 & 0.5027 & 0.2164 \\
\bottomrule
\end{tabular}
\end{table}


==> figs/output_tables/4_2_cross_model_rst.tex <==
\begin{table}[h]
\centering
\caption{Impacts By Crossing Explicit Conditions of Models}
\label{tab:crossModel}
\begin{tabular}{rrrrr}
\toprule
{} & {} & {HHAR} & {WHAR} & {TAPRINT} \\
\midrule
\multirow[t]{3}{*}{$DA^\ast$} & 5NN & 0.8066 & 0.5350 & 0.5107 \\
 & MetaSense & 0.8748 & 0.7854 & 0.6242 \\
 & CrossValid. & 0.9000 & 0.8727 & 0.7863 \\
\multirow[t]{2}{*}{w/o DA} & 5nn & \underline \bfseries 0.6973 & \underline \bfseries 0.5325 & 0.3219 \\
 & MetaSense & 0.7206 & 0.7141 & \underline \bfseries 0.2378 \\
\bottomrule
\end{tabular}
\end{table}

